SAPE: Spatially-Adaptive Progressive Encoding for Neural Optimization

Multilayer-perceptrons (MLP) are known to struggle with learning functions of high-frequencies, and in particular cases with wide frequency bands. We present a spatially adaptive progressive encoding (SAPE) scheme for input signals of MLP networks, which enables them to better fit a wide range of frequencies without sacrificing training stability or requiring any domain specific preprocessing. SAPE gradually unmasks signal components with increasing frequencies as a function of time and space. The progressive exposure of frequencies is monitored by a feedback loop throughout the neural optimization process, allowing changes to propagate at different rates among local spatial portions of the signal space. We demonstrate the advantage of SAPE on a variety of domains and applications, including regression of low dimensional signals and images, representation learning of occupancy networks, and a geometric task of mesh transfer between 3D shapes.

==> 08_broader_impact.tex <==
\section*{Broader impact}

SAPE is a method for boosting the accuracy of learned implicit neural functions. It can be leveraged to enable new applications or improve various downstream tasks that involve precise processing of signals, like segmentation, or reconstruction of complex signals, such as streaming video or Signed Distanced Functions. Beyond the domains of vision and graphics, we conjecture SAPE might also benefit applications in speech \& audio, and signal processing in general. Depending on their use, all mentioned applications may have positive or potentially negative impact. SAPE can be used to facilitate novel applications that require accurate recovery of signals, like 3D reconstruction for AR and VR. It can also be misused for the purpose of generating fake media, including audio, video and images.

==> algorithms/sape_algo.tex <==
\begin{algorithm}[H]
\DontPrintSemicolon
\SetAlgoLined
\SetKwInput{KwResult}{Hyperparameters}
\SetKwInput{KwData}{Input}
\KwResult{Coordinates mapping function $E: \mathbb{R}^{d} \mapsto \mathbb{R}^{n}$, \\
Encoding-weights grid resolution ${g_r}^d$, Weight progression policy $\Phi$, Convergence threshold $\varepsilon$}
\KwData{Samples of coordinates $\mathbf{p} \in \mathbb{R}^{d}$, Corresponding signal values $\mathbf{y} \in \mathbb{N}$.}
\Indp
 randomly initialize network weights $\bm{\theta}_0$. \;
 initialize encoding weights $\bm{\alpha}_{0} \in {g_{r}}^{d}$. \;
 
 \For{training step $t \in T $}{
 \tcc*[h]{Obtain encoding mask per interpolated grid weights by $\mathbf{p}$} \;
 $\bm{\alpha}_{t}[\mathbf{p}] \longleftarrow interpolate_{\bm{\alpha}_{t}}(\mathbf{p}) $ \;
  $\mathbf{x}_t \longleftarrow {\bm{\alpha}_{t}[\mathbf{p}]}^{\top} E(\mathbf{p})$ \tcc*[h]{Map coordinates to network input} \;
  $\hat{\mathbf{y}}_t \longleftarrow f_{\theta}(\mathbf{x}_t)$ \tcc*[h]{Obtain network prediction, per coordinate $\mathbf{p}$} \;
  
  \For{grid coordinate $g_p \in {g_r}^d $}{
  \tcc*[h]{If weighted grid coordinate loss is above threshold} \;
    \If{$\mloss (\hat{\mathbf{y}}_{t}, \mathbf{y}) \ge \varepsilon$}{
    \tcc*[h]{Increase weight for encoding frequencies} \;
    $\bm{\alpha}_{t+1}[\mathbf{p}] \longleftarrow \Phi(\bm{\alpha}_{t}[\mathbf{p}])$ \;
    } 
  }
    $ \bm{\theta}_{t+1} \longleftarrow \bm{\theta}_{t} - \beta \nabla_{\bm{\theta}_{t}} \mloss{}(\hat{\mathbf{y}}_t, \mathbf{y}) $ \;  
 }
 \caption{SAPE Algorithm}
\end{algorithm}


==> figures/04_occupancies.tex <==
\begin{figure}
\begin{overpic}[width=\textwidth,tics=10]{figures/04_occupancies.png}

\put(7,-2.5){\scriptsize{Ground truth}}
\put(26, -2.5){\scriptsize{No encoding}}
\put(49, -2.5){\scriptsize{FF}}
\put(69, -2.5){\scriptsize{Siren}}
\put(86, -2.5){\scriptsize{SAPE + FF}}
\end{overpic}
\vspace{2pt}
\caption{3D Occupancy network task. \dc{if we are exactly the same as siren, use only the two rows in the middle.}}

\label{fig:occupancies}

\end{figure}

==> figures/04_occupancies2.tex <==
\begin{figure}
\begin{overpic}[width=\textwidth,tics=10]{figures/04_occupancies2.png}

\put(5,1){\scriptsize{Ground truth}}
\put(25,1){\scriptsize{No encoding}}
\put(48, 1){\scriptsize{Siren}}
\put(68, 1){\scriptsize{FF}}
\put(85, 1){\scriptsize{SAPE + FF}}
\end{overpic}
\vspace{2pt}
\caption{3D Occupancy. }

\label{fig:occupancies2}

\end{figure}

==> figures/04_spatially_adaptive.tex <==
\begin{figure}
\begin{overpic}[width=\textwidth,tics=10]{figures/04_spatially_adaptive.jpg}

\put(-6, 18.5){\rotatebox{90}{\parbox{.7in}{\centering{\small{Spatially Adaptive}}}}}
\put(-6, 5){\rotatebox{90}{\parbox{.7in}{\centering{\small{Non-Spatially Adaptive}}}}}

\put(14, 2){\small{\textit{Enlarged output areas}}}
\put(56, 2){\small{\textit{Ground Truth}}}
\put(75.5, 2){\small{\textit{Cutoff Frequency Heatmap}}}

\put(73, 32.5){\small{$low$}}
\put(98, 32.5){\small{$high$}}




\end{overpic}
\caption{Comparison of SAPE with a spatial adaptive grid (top left) and without it (bottom left). The spatial adaptive variant leverages high frequencies only in image areas which require it: the heatmap to the right indicates the maximal frequency unmasked in each of the $256 \times 256$ grid coordinates. Masking excess encoding dimensions in smooth areas allows the network to better fit high frequency areas. Details such as tiny holes, grains of sand and apexes of leaves are now clearly visible.
Please zoom in to examine the differences.}
\label{fig:spatial_adaptive}

\end{figure}

==> figures/04_zebra_sample.tex <==
\begin{figure}
\begin{overpic}[width=\textwidth,tics=10]{figures/04_zebra_sample.pdf}


\put(0, 22){\scriptsize{SAPE}}
\put(0, 9){\scriptsize{FFN}}
\put(0, 0){\scriptsize{Sample rate}}

\put(10.5, 0){\scriptsize{$5\%$}}
\put(23, 0){\scriptsize{$15\%$}}
\put(36.8, 0){\scriptsize{$25\%$}}
\put(49.8, 0){\scriptsize{$35\%$}}

\put(78, 1){\scriptsize{Pixels Sample Rate}}
\put(59,13.5)
{\begin{turn}{90} \scriptsize{PSNR}\end{turn}}



\end{overpic}
\caption{2D image regression over increasing size of sample rate training pixels. Our method is adaptive for different number of training samples while FFN ($\sigma=15$) struggles as the pixels sample rate decreases. }
\label{fig:sample_rate}

\end{figure}

==> tables/tab_images.tex <==
\begin{table}
\centering

\begin{tabular}{l  c c}
\toprule
 & \textbf{Natural Images} & \textbf{Text Images} \\
\midrule
No Encoding & $19.72 \pm 2.77$ & $19.39 \pm 2.02$\\ 
Siren & $27.03 \pm 4.28$ & $30.81 \pm 1.72$\\ 
RBFG & $25.98 \pm 3.98$ &  \\
P-RBFG & $ 27.06 \pm 3.94 $&\\
FF & $25.57 \pm 4.19$ & $30.47 \pm 2.11$\\

P-FF &  $\boldsymbol{28.09 \pm 4.04}$ & $\boldsymbol{31.84 \pm 2.15}$\\
\bottomrule

\end{tabular}
\caption{TODO: PSNR of images (2d image regression)}
\label{tab:images}

\end{table}
 
